Computing $L(p,1)$-Labeling with Combined Parameters

Given a graph, an $L(p,1)$-labeling of the graph is an assignment $f$ from the vertex set to the set of nonnegative integers such that for any pair of vertices $(u,v),|f (u) - f (v)| \ge p$ if $u$ and $v$ are adjacent, and $f(u) \neq f(v)$ if $u$ and $v$ are at distance $2$. The $L(p,1)$-labeling problem is to minimize the span of $f$ (i.e.,$\max_{u\in V}(f(u)) - \min_{u\in V}(f(u))+1$). It is known to be NP-hard even for graphs of maximum degree $3$ or graphs with tree-width 2, whereas it is fixed-parameter tractable with respect to vertex cover number. Since vertex cover number is a kind of the strongest parameter, there is a large gap between tractability and intractability from the viewpoint of parameterization. To fill up the gap, in this paper, we propose new fixed-parameter algorithms for $L(p,1)$-Labeling by the twin cover number plus the maximum clique size and by the tree-width plus the maximum degree. These algorithms reduce the gap in terms of several combinations of parameters.

==> Relabeling.tex <==
\begin{lemma}
\label{lem:tc:I_i}
%Let $n_i$ be the number of vertices of $I_{i}(\forall i=1, 2, \ldots, s)$ and the maximum clique size be $\omega _i$. 
Suppose that each $T_i$ satisfies $\omega _i\le \frac{n_{i}}{2}$.
Then, any $L(2,1)$-labeling of $G$ can be transformed into an $L(2,1)$-labeling of $G$ such that each $T_i$ uses  $n_i$ labels.

%there is an $L(p,1)$-labeling any $n_i$ label can be assigned to $T_i$ satisfying the \textsc{$L(2,1)$-Labeling} constraint. 
%$I_{i}(\forall i=1, 2, \ldots , s)$の頂点数を$n_i$, 最大クリークサイズを$\omega _i$とすると, $\omega _i\le \frac{n_{i}}{2}$であるとき, 任意の$n_i$種類のラベルで\textsc{$L(2,1)$-Labeling}制約を満たす$I_i$へのラベル割当が可能である. 
\end{lemma}
\begin{proof}
We are given an  $L(2,1)$-labeling $f$ of $G$.
Suppose that $T_i$ uses $k$ labels $l_1, l_2, \ldots, l_k$ where $l_1\le l_2\le \ldots\le  l_k$.
Because each vertex in $T_i$ has the common neighbor in $X$, the number $k$ of labels  is at least $n_i=|T_i|$.

If $k = n_i$, we are done.
Otherwise, we relabel vertices in $T_i$ using only $l_1, l_2, \ldots, l_{n_i}$.
Because $f$ is an $L(2,1)$-labeling, every vertex within distance 2 from $T_i$ does not use any of $l_1, l_2, \ldots, l_k$. Moreover, the labels used by neighbors of $T_i$ is at least 2 apart from each of them.
Thus, this relabeling does not affect vertices not in $T_i$.

The relabeling is simple. 
%Let $C_1, \ldots, C_{\ell}$ be cliques of type $T_i$ where $\omega_i=|C_1|\ge \ldots \ge |C_{\ell}|$. Note that $|\bigcup_{i=1}^{\ell}C_i| = n_i$.
If $n_i$ is odd, we label each clique in decreasing order of size by using labels in order of $l_1, l_3, \ldots, l_{n_i}, l_2, l_4,  \ldots, l_{n_{i-1}}$, and otherwise, we label them in order of $l_1, l_3, \ldots, l_{n_i-1}, l_2, l_4,  \ldots, l_{n_{i}}$.
Due to $\omega _i\le \frac{n_{i}}{2}$, the relabeling satisfies the condition of $L(2,1)$-labeling and it uses exactly $n_{i}$ labels. By relabeling cliques for every $T_i$, we can obtain an $L(2,1)$-labeling of $G$ such that such that each $T_i$ uses  $n_i$ labels.\qed


% Arrange $n_i$ labels in ascending order of value. After that, rearrange so that even-numbered labels are arranged after odd-numbered labels (in order of $1$st, $3$rd, \ldots, $2$nd, $4$th, \ldots). These sorted labels are assigned in descending order of clique size. 
% The label difference may be less than $2$ only when the labels are adjacent in ascending order. 
% Therefore, it can be said that the constraint is not violated unless adjacent labels are assigned to the same clique. 
% That is, when arranged in ascending order from the odd-numbered first, consecutive $\lceil \frac{n_i}{2}\rceil-1$ labels apart $2$ or more in any value. 
% In particular, it holds from the first value to $\lceil \frac{n_i}{2}\rceil$ labels and the subsequent $\lfloor \frac{n_i}{2}\rfloor$ labels. 
% Therefore, by performing this assignment, it can be said that if $\omega _i\le \frac{n_{i}}{2}$, it is possible to satisfy the \textsc{$L(2,1)$-Labeling} constraint in $T_i$. 
%直訳
%$n_i$個のラベルを値が昇順になるよう並べる. 
%その後, 奇数番目のラベルの後ろに偶数番目のラベルが並ぶよう並べ替え($1番目,3番目,\ldots, 2番目,4番目,\ldots$の順), 
%このように並べ替えたラベルをクリークサイズの大きいものから順に割り当てる. 
%昇順に並べた際, ラベルが隣り合う場合のみラベル差が$2$未満である可能性がある。従って同じクリークに対して隣り合うラベルを割り当てなければ制約を違反しないといえる.

%$n_i$個のラベルを値が昇順になるよう並べ, 奇数番目のラベルののち, 偶数番目のラベルが並ぶよう並べ替え($1番目,3番目,\ldots, 2番目,4番目,\ldots$の順), クリークサイズの大きいクリークから並べ替えたラベルを順に割り当てる. 
%このとき, 昇順に並べた際の$x$番目の値と差が$2$未満である可能性があるのは$x-1$もしくは$x+1$番目の値のみであり, 同じクリークに割り当てるラベルは前後するラベルを割り当てなければ制約を違反しないといえる. 
%従って, 昇順の奇数番目から先に並べることで連続する$\lceil \frac{n_i}{2}\rceil - 1$個のラベルはどの値同士も差が$2$以上であり, 特に初めの値から$\lceil \frac{n_i}{2}\rceil$個, それ以降の$\lfloor \frac{n_i}{2}\rfloor$個のラベルにおいても成り立つ. 
%これより上記のラベル順で最大クリークから順に割り当てを行うことで $\omega _i\le \frac{n_{i}}{2}$であれば$T_i$内に関して\textsc{$L(2,1)$-Labeling}制約を満たす割当が可能であるといえる. 
\end{proof}




\color{black}


\begin{lemma}
\label{lem Xlabel}
Suppose that each $T_i$ satisfies $\omega_i \le \frac{n_i}{2}$.
Then one can transform any $L(2,1)$-labeling $f$ of $G$ into an $L(2,1)$-labeling $f'$ so that $X$ uses only labels in $\{0,1,\ldots, 4\tc -2\} \cup \{\lambda -4\tc +2, \ldots, \lambda \}$. 
%When $\omega_i \le \frac{n_i}{2} (\forall i=1, 2, \ldots ,s)$, it is possible to change any label assignment to $G$ that satisfies the \textsc{$L(2,1)$-Labeling} constraint so that $X$ is assigned only in the $\{0,1,\ldots, 4\tc -2\} \cup \{\lambda -4\tc +2, \ldots, \lambda \}$ label range. 
%$\omega_i \le \frac{n_i}{2} (\forall i=1, 2, \ldots , s)$のとき, \textsc{$L(2,1)$-Labeling}制約を満たす$G$への任意のラベル割当を$X$への割当がZZのラベル範囲でのみ行われる割り当てに変更が可能である. 
\end{lemma}
\begin{proof}
Let $a,b\in \{0, 1, \ldots, \lambda \}$ be two labels that are not used in $X$ and at least $2$ apart from all the labels used in $X$. 
Without loss of generality, we assume $a\le b$.
Then, for each label between $a$ and $b$, we change the labels as follows.
%$X$の頂点に割り当てられているすべてのラベルと少なくとも$2$の差があるラベル$a,b\in \{0, 1, \ldots, \lambda \}$を考える. 
%ラベルを以下の操作に従い置き換える. 
% \begin{align*}
% f & & f'\\
%     a &\rightarrow & a+1 \\
%     a+1 &\rightarrow &a+2 \\
%     &\vdots& \\
%     b &\rightarrow &a \\
% \end{align*}

\begin{table}[h]
\centering
\scalebox{1.2}{
  \begin{tabular}{ccc}
    %$f$ & & $f'$\\
    $a$ &$\rightarrow$ & $a+1$ \\
    $a+1$ &$\rightarrow$  &$a+2$ \\
    &$\vdots$& \\
    $b$ &$\rightarrow$  &$a$ \\
  \end{tabular}
  }
\end{table}

We notice that only labels in $\{a+2, \ldots, b-2\}$ are changed in $X$.
%so $3$ labels that are at most $1$ offset from the label of any vertex of $X$ are either all reassigned or all unchanged. 
%Because labels $a$ $b$ is at least 2 different from any label for $X$
Therefore, the new labeling satisfies the condition of $L(2,1)$-labelings in $G[X]$.

%Therefore, the label difference between any vertices of $X$ does not become less than $2$, so the \textsc{$L(2,1)$-Labeling} constraint violation does not occur between vertices of $X$. 
Next, we show that the new labeling is an $L(2,1)$-labeling in $G$.
To show this, we consider three cases with respect to $V\setminus X$.

%このとき, $X$では$a+2 , \ldots, b-2$までのラベルにおいてのみ置き換えが起こり, $X$の任意の頂点のラベルから高々$1$ずれた$3$つのラベルは, すべて置き換えられるかすべて変わらないかのどちらかであることに注意されたし. 
%よって$X$のどの頂点間でのラベル差も$2$以下にならないため, $X$の頂点間では\textsc{$L(2,1)$-Labeling}制約違反が起こらない. 
%次に, $X$の頂点と$I$の頂点間におけるラベル制約にも違反が起こりえないことを説明する. 
\begin{description}
\item[Case $1$. Labels of $V\setminus X$ in $\{0,1, \ldots, a-1\}\cup \{b+1, \ldots, \lambda \}$. ]
\

In this case, the labels of vertices in $V\setminus X$ are not changed.
Since  only labels $a+2, \ldots, b-2$ in $X$ are changed to $a+3, \ldots, b-1$ and labels in $\{0,1, \ldots, a-1\}\cup \{b+1, \ldots, \lambda \}$ are at least 2 different from $a, a+1, \ldots, b-1$, the new labeling does not violate the condition of  $L(2,1)$-labelings.

% Since there is no label replacement and it does not interfere with the label of $X$, the constraint violation does not occur (because in $X$, the replacement occurs only up to $a+2, \ldots, b-2$ labels). 
%\item[$I$のラベルが$\{0,1, \ldots, a-1\}$, $\{b+1, \ldots, \lambda \}$のとき]\mbox{}\\
%ラベルの置き換えがなく, $X$のラベルとも干渉しないため違反は起こりえない($X$では$a+2 , \ldots, b-2$までのラベルにおいてのみ置き換えが起こるため). 
\item[Case $2$. Labels in  $\{a, \ldots, b-1 \}$. ]\mbox{}\\
The label difference between $I$ and $X$ may be narrowed when the label of $X$ is $\{b, b+1, \ldots, \lambda\}$. 
In particular, the label difference can be less than $2$ only when the label of $X$ is $\{b, b+1\}$. 
However, since the label $\{b, b+1\}$ is not assigned to $X$ by the condition, the constraint violation cannot occur. 
%\item[$I$のラベルが$\{a, \ldots, b - 1 \}$のとき]\mbox{}\\
%$I$と$X$とのラベル差が狭まる可能性があるのは$X$のラベルが$\{b, b+1, \ldots, \lambda\}$のときである.  
%特にラベル差が$2$以下になり得るのは$X$のラベルが$\{b, b+1\}$のときのみである. 
%しかし条件より$X$にはラベル$\{b, b+1\}$が割り当てられていないため制約違反は起こりえない. 
\item[Case $3$. The label of $I$ is $\{b\}$. ]\mbox{}\\
Since the label of $\{a-1, a, a+1\}$ is not assigned in $X$, even if the label in $I$ changes to $a$, the difference between the label in $I$ and the label in $X$ is more than $2$. Therefore, constraint violation cannot occur. 
%\item[$I$のラベルが$\{b\}$のとき]\mbox{}\\
%\ $X$内には$\{a-1, a, a+1\}$のラベルは割り当てられていないため, ある$I$のラベルが$a$に変わったとしても$I$内と$X$内のどのラベルとの差も$2$以上である. 従って制約違反は起こりえない. 
\end{description}
The label constraint between vertices in $I$ is explained. From the condition, the original label assignment does not assign the same label in the same $I_i$, and the replacement is performed in a loop, so the same label is not assigned in the same $I_i$ after reassignment. Therefore, by reassigning the label for each $I_i$ using the lemma \ref{lem:tc:I_i}, we can always obtain an assignment that does not violate the constraint. 
%$I$における頂点間のラベル制約について説明する. 条件より元のラベル割当では同じ$I_i$内で同じラベルが割り当てられることがなく, 置き換えがループで行われるため, 置き換え後も同じラベルが同じ$I_i$内の別頂点に割り当てられることがないといえる. 従って, 補題\ref{lem:tc:I_i}を用いた各$I_i$に対するラベルの再割り当てを行うことで制約に違反しない割り当てを必ず求めることができる. 
%また, $I$における頂点間のラベル制約については, 元のラベル割当でも同じ$I_i$内で別頂点に同じラベルが割り当てられることがなく, 置き換えがループで行われるため, 置き換え後も同じラベルが別頂点に割り当てられることがないといえる. 従って, 補題\ref{lem:tc:I_i}を用いて各$I_i$にて再割り当てを行うことで制約に違反しない割り当てを必ず求めることができる. 

By repeating the above operation, the difference between adjacent labels used in $X$ can be reduced to at most $3$. 
At the time when this operation became impossible, the maximum value of $\tc$ labels assigned to $X$ was $3\tc-2$ when it was moved to the smallest possible value (This label assignment is in ascending order $\{1,4,\ldots, 1 + 3(\tc-1)\}$). 
And the minimum value was $\lambda - 3\tc + 2$ when it was moved to the biggest possible value (This label assignment is in ascending order $\{ \lambda-1-3(\tc-1), \ldots, \lambda-4, \lambda-1\}$). 
Therefore, one can assign labels to $X$ in the range $\{0,1,\ldots, 4\tc -2\} \cup \{\lambda -4\tc +2, \ldots, \lambda \}$. \qed
%上記の操作を繰り返すことで$X$で使用される隣り合ったラベルの差を高々$3$にすることができ, 操作不可能となった時点での$\tc$個のラベルは, 小さい値にすべて寄った場合でも最大値は高々$3\tc - 2$\ (この時のラベル割当は昇順で$\{1,4,\ldots, 1 + 3(\tc - 1)\}$となるため). 大きい値にすべて寄った場合でも最小値は$\lambda - 3\tc + 2$\ (この時のラベル割当は昇順で$\{ \lambda - 1 - 3(\tc - 1), \ldots, \lambda - 4, \lambda - 1\}$となるため). 従って$\{0,1,\ldots, 4\tc -2\} \cup \{\lambda -4\tc +2, \ldots, \lambda \}$の範囲で$X$へのラベル割当が可能だといえる. 
\end{proof}


==> clique_width.tex <==
\section{Parameterization by $\cw + \Delta$}\label{sec:cliquewidth}
As \textsc{$L(p,1)$-Labeling} is paraNP-hard for tree-width, so is for clique-width.  
%NP-hard even on graphs of tree-width 2, and hence it is paraNP-hard for tree-width.
%This also implies that \textsc{$L(2,1)$-Labeling} is paraNP-hard for clique-width.
In this section, as a complement,
we show that \textsc{$L(p,1)$-Labeling} (actually, \textsc{$L(p,q)$-Labeling} for any constant $p$ and $q$) is fixed-parameter tractable when parameterized by $\cw + \Delta$.

To show this, we give a one-sorted monadic-second order logic (MSO$_1$) representation of \textsc{$k$-$L(p,q)$-Labeling}.
% We first define the following formula $\distmso_{\le 2}(u,w)$, which is true if the distance between $u$ and $w$ is at most $2$:
% \begin{align*}
%     \distmso_{\le d}(u,w):=\exists v_0, \ldots, v_d: (v_0=u) \land (v_2=w) \land \left(\bigwedge_{0\le i \le d}(v_i\neq v_{i+1}) \lor \adj(v_i,v_{i+1})\right) 
% \end{align*}
We first define the following formula $\distmso_{=2}(u,w)$, which is true if the distance between $u$ and $w$ is exactly $2$:
\begin{align*}
    \distmso_{=2}(u,w):= &(u\neq w) \land \lnot \adj(u,w)\\ 
    & \land  (\exists v\in V: (u\neq v)  \land  (v\neq w) \land (\adj(u,v)\land \adj(v,w) ).
    % \distmso_{=2}(u,w):=\exists v_0, v_1, v_2: & (v_0=u) \land (v_2=w) \land \left(\bigwedge_{0\le i<j\le2}v_i\neq v_j\right) \\
    % &\land (\adj(v_0,v_1)\land \adj(v_1,v_2) \land \lnot \adj(v_0,v_2)) 
\end{align*}
Then the formula $\varphi_{k}$ such that $G\models \phi_{k}$ if and only if $(G, k)$ is a yes instance of \textsc{$L(p,q)$-Labeling} is defined as follows:
\begin{align*}
    \varphi_{k}:=&\exists V_0,\ldots, V_{k}: \left(\forall v: \bigvee_{0\le i\le k}(v\in V_i \land \bigwedge_{0\le j\neq i\le k}v\notin V_j)\right)\\ 
    &\land (\forall u,v:\adj(u,v)\Rightarrow 
    \bigvee_{0\le i\le k}(u\in V_i \land (\bigwedge_{i-p+1\le j\le i+p-1} v\notin V_j)) )\\
     &\land \left(\forall u,v: (\distmso_{= 2}(u,v))\Rightarrow  \bigvee_{0\le i\le k} (u\in V_i \land (\bigwedge_{i-q+1\le j\le i+q-1} v\notin V_j)) \right).
\end{align*}

For a graph $G$ of clique-width at most $\cw$ and for an MSO$_1$ formula $\psi$, it can be checked whether $G\models \psi$ in time $O(g(|\psi|,\cw)\cdot n^3)$, where $g$ is some computable function \cite{Courcelle2000,Oum2008}.
Because the length of MSO$_1$ formula $\varphi_{k}$ depends on $k$, $p$, and $q$, \textsc{$k$-$L(p,q)$-Labeling} is fixed-parameter tractable when parameterized by $k+\cw$.
Thus, we obtain the following theorem.

\begin{theorem}
For any fixed $p,q$, \textsc{$L(p,q)$-Labeling} is fixed-parameter tractable when parameterized by $\lambda_{p,q}+\cw$.
\end{theorem}

As for the labeling number, since the degree of $G^2$ is $\Delta^2$, $\lambda_{1,1}(G) \le \Delta(G)^2$ holds. This and $\lambda_{cp,cq}=c\lambda_{p,q}$ (\cite{Georges1995GeneralizedVL}) imply that  
$\lambda_{p,q}\le \max\{p,q\}\Delta^2$ holds. For $q=1$, a better bound $\lambda_{p,1}\le \Delta^2+(p-1)\Delta-2$ is known~\cite{Goncalves2008}. 
Thus we have the following corollary. 

%Since $\lambda_{p,1}\le \Delta^2+(p-1)\Delta-2$ holds for any graph $G$ \cite{Goncalves2008}, we have the following corollary. 
\begin{corollary}
For any positive constant $p$ and $q$, \textsc{$L(p,q)$-Labeling} is fixed-parameter tractable when parameterized by $\Delta+\cw$.
\end{corollary}

